Active choice of teachers, learning strategies and goals for a socially guided intrinsic motivation learner

We present an active learning architecture that allows a robot to actively learn which data collection strategy is most efficient for acquiring motor skills to achieve multiple outcomes, and generalise over its experience to achieve new outcomes. The robot explores its environment both via interactive learning and goal-babbling. It learns at the same time when, who and what to actively imitate from several available teachers, and learns when not to use social guidance but use active goal-oriented self-exploration. This is formalised in the framework of life-long strategic learning. The proposed architecture, called Socially Guided Intrinsic Motivation with Active Choice of Teacher and Strategy (SGIM-ACTS), relies on hierarchical active decisions of what and how to learn driven by empirical evaluation of learning progress for each learning strategy. We illustrate with an experiment where a simulated robot learns to control its arm for realising two kinds of different outcomes. It has to choose actively and hierarchically at each learning episode: 1) what to learn: which outcome is most interesting to select as a goal to focus on for goal-directed exploration; 2) how to learn: which data collection strategy to use among self-exploration, mimicry and emulation; 3) once he has decided when and what to imitate by choosing mimicry or emulation, then he has to choose who to imitate, from a set of different teachers. We show that SGIM-ACTS learns significantly more efficiently than using single learning strategies, and coherently selects the best strategy with respect to the chosen outcome, taking advantage of the available teachers (with different levels of skills).

==> SGIMACTSalgorithm/PseudoCodeActionsInterest.tex <==
\begin{algorithmbis}[\textsf{ [mLow] = Low Level: Goal-Directed Actions Interest Computation}]\label{alg:PseudoCodeActionsInterest}
\begin{algorithmic}
	        \STATE{Search in $Memo$ for the  $y_{close}$ closest to $y_g$}
	        \STATE{ $mLow \gets$  mode \textit{global-exploration} or \textit{local-optimization} with probability   $\propto Sim(y_{close} y_g)$}
	        \RETURN{mLow}
	        
\end{algorithmic}
\end{algorithmbis}	        

==> SGIMACTSalgorithm/PseudoCodeExecute.tex <==

\begin{algorithmbis}[\textsf{ [$Memo,y$] = Execute}($c, a$) \\ Set context $c$ and perform action parameters $a $ ] \label{alg:Execute}
\begin{algorithmic}
\STATE{ Initialise robot at $c $  }
\STATE{Perform action of parameters $a$.}
\STATE{Measure state y in the task space} 
\STATE{Update $Memo$ with $(c, a,y) $ }	  
\STATE{$flagInteraction  \gets $ check for a teacher's demonstration}
\RETURN  $Memo, y$
\end{algorithmic}
\end{algorithmbis}


==> SGIMACTSalgorithm/PseudoCodeExploration.tex <==
 \begin{algorithmbis}[\textsf{[$Memo$] = Decide an Action($c,y_g$) \\ Search for actions to reach $y_g$ in context $c$ while building model}] 
 \label{alg:PseudoCodeExploration}
\begin{algorithmic}
   \STATE{Search in $Memo$ for the  $y_{close}$ closest to $y_g$}
	        \STATE{ $mLow \gets$  mode \textit{global-exploration} or \textit{local-optimization} with probability   $\propto Sim(y_{close}, y_g)$}
  \IF{ $mLow$ =  \textit{global-exploration} }
	        \STATE{Action parameter $a \gets$  random movement parameters}
	       % \STATE{ Initialise robot at $(x_{org},y_{org}) $ }
	        \STATE{$[Memo,y] \gets $  \textsf{ Execute}($c, a$)}
	       % \STATE{Measure new state $(x_2,y_2)$  and memorise $(x_{org},y_{org}, a,x_2,y_2)$ }
	  \ELSIF{ $mLow$ =   \textit{local-optimization}}
	     \STATE{\textsf{LocalOptimization}($c,y_g$) }
	  \ENDIF
\RETURN{$Memo$}
\end{algorithmic}
\end{algorithmbis}

==> SGIMACTSalgorithm/PseudoCodeImitation.tex <==
 \begin{algorithmbis}[\textsf{ [Memo] = Imitate Action($a_{demo},c$)}] \label{alg:PseudoCodeImitation}
\begin{algorithmic}
\STATE {{\bfseries Input:} $nIm$ : duration of the imitation phase;}
\STATE {{\bfseries Input:} thresholds:  $\epsilon_{max}$; }

  	\FOR{$nbImitate$ times}
	\STATE{$a_{rand} \gets$  random vector such that $|a_{rand}|< \epsilon_{max}$}
	\STATE{$a \gets a_{demo} + a_{rand}$  }
	\STATE{$Memo,y \gets $ \textsf{ Execute} ($c,a$)}
	\ENDFOR
\RETURN{Memo}
\end{algorithmic}
\end{algorithmbis}

==> SGIMACTSalgorithm/PseudoCodeLocalData.tex <==
\begin{algorithmbis}[\textsf{ [$K_{l_{best}} $] = LocalData}($ y_g,Memo$) \\ Retrieve from the memory $Memo$ experiences in the locality of $y_g$  ] \label{alg:LocalData}
\begin{algorithmic}
\STATE{ {\bfseries input}: thresholds distM, distN, $\sigma$ }
\STATE{Get from the memory the nearest neighbours of $y_g$: }
\STATE{$ L \gets \{(a_l,y_l) \in Memo |  \left\{
\begin{array}{rl}
Sim(y_l,y_g) <distM\\
Sim(y_l,y_g) < Sim(y,y_g) , \forall (a,y) \in Memo - L\\ 
 \end{array} \right.
 \} 
 $}
\STATE{$\forall (a_l,y_l) \in L$, $K_l \gets \{(a,y)\in Memo| ||a-a_l|< distN \} $ }
\STATE{Select the best locality :$ l_{best} \gets argmin(\textsf{LocalQuality}(K_l,y_g) $}
\RETURN{ $K_{l_{best}} $}
\end{algorithmic}
\end{algorithmbis}


==> SGIMACTSalgorithm/PseudoCodeLocalOptimization.tex <==
\begin{algorithmbis}[ \textsf{ LocalOptimization}($c_g,y_g$) \\ Optimisation to minimise  $Sim( (c,y),(c_g,y_g)) $ with respect to the action parameters $a$ so that $M: (c, a) \mapsto y$]\label{alg:optimisation}
\begin{algorithmic}

\STATE{{\bfseries input}: $n$ : dimension of A .}
\STATE{ $\{s_i = (c_i, a_i),  \forall i=1..n+1 \} \gets $ \textsf{LocalData}($c_g,y_g$)}
\LOOP
	\STATE{Order the points in the simplex from lowest value $f(s_1)$ to highest $f(s_{n+1})$. }
	\STATE{\underline{At each step in the iteration, the algorithm discards the current worst point $s_{n+1}$,}  \underline{and accepts another point into the simplex.}}
	\STATE{Generate the reflected point $r = (c_r,a_r)\gets 2m - s_{n+1}$,  where  $m = \frac{ \sum s_i}{n}, i = 1...n$.}
	\STATE{ \textsf{Execute} $(c_r,a_r)$ and measure $f(r)$.}
	\IF{ $f(s_1) \leq f(r) < f(s_n)$ }
		\STATE{ $s_{n+1} \gets r$ and terminate this iteration.}
	\ELSIF{ $f(r) < f(s_1)$}
		\STATE{ Calculate the expansion point u: $u =(c_u, a_u) \gets m + 2(m - s_{n+1})$.}
		\STATE{\textsf{Execute} $(c_u, a_u)$ and calculate $f(u)$.}
		\IF{ $f(u) < f(r)$}
			\STATE{ $s_{n+1} \gets u$ and terminate the iteration.}
		\ELSE
		\STATE{ $s_{n+1} \gets r$ and terminate the iteration.}
		\ENDIF
	\ELSIF{ $f(r) \geq f(s_n)$}
		\STATE{ \underline{Perform a contraction between $m$ and  the better of $s_{n+1}$ and $r$}}
		\IF{ $f(r) < f(s_{n+1})$ (i.e. r is better than $s_{n+1}$),}
			\STATE{Calculate  $k =(c_k, a_k) \gets m + (r - m)/2$ .}
			\STATE{\textsf{Execute} $(c_k, a_k)$ and measure $f(k)$.}
			\IF{$ f(k) < f(r)$}
				\STATE{ $s_{n+1} \gets k$ and terminate the iteration.}
			\ELSE
			\STATE{ Continue with Step \textsf{New Simplex}. }
			\ENDIF
			
		\ELSIF{ $f(r) \geq f(s_{n+1})$}
			\STATE{ $h \gets m + (s_{n+1} - m)/2 $.}
			 \STATE{ \textsf{Execute}$(c_h, a_h)$ and measure $f(h)$.}
			\label{aa}
			\IF{ $f(h) < f(s_{n+1}$)}
			\STATE{ $s_{n+1} \gets h$ and terminate the iteration.}
			\ELSE
			\STATE{ Continue with Step  \textsf{New Simplex} .}
			\ENDIF
			
		\ENDIF
	\ENDIF

\label{aaa}	
\STATE{Step \textsf{New Simplex:} $ v_i=(c_{v_i,}a_{v_i})  \gets s_1 + \frac{s_i  - s_1}{2} , i = 2,...,n+1$.}
\STATE{\textsf{Execute}$(c_{v_i,}a_{v_i}) $ and calculate $f(v_i), i = 2,...,n+1$. }
\STATE{The simplex at the next iteration is $s_1, v_2,...,v_{n+1}$. }
\ENDLOOP

\end{algorithmic}
\end{algorithmbis}



==> SGIMACTSalgorithm/PseudoCodeSGIMA.tex <==
\begin{algorithmbis}[Pseudo-Code of SGIM-A]\label{alg:PseudoCodeSGIMA}
\begin{algorithmic}
\STATE {{\bfseries Input:} $nbImitate$ : duration of the imitation phase;}
\STATE {{\bfseries Input:} thresholds:  $\epsilon_{max}$; }
%\STATE {\bfseries Initialization:} rest position $(x_{org}, y_{org})$.
\STATE {\bfseries Input:} $p_1, p_2, p_3$ as probabilities of methods for choosing a goal in the task space by the Goal Self-Generation Module (totally random, random goal in the most interesting region, worst mastered goal in the most interesting region)  
\STATE  {\bfseries Initialization:} $\mathcal{R } \gets $  singleton ${C \times Y}$, $Memo \gets$  empty episodic memory


\LOOP

       \STATE{\textbf{\underline{High Level of Active Learning : Module 2 Goal Self-Generation}}}
       \STATE{Measure current configuration $c$}	
       \STATE{Using mode $m \in {[1;2;3]}$ with probability $p_m$, select  a region $R_n  \in \mathcal{R}$ and a goal $y_g$ so that $(c,y_g) \in R_n$ }
       \STATE{$\gamma \gets $ estimate competence of $(c,y_g)$.}
       \IF {$\gamma > y_m$}
           \STATE{{\underline{Low Level : Goal Directed Exploration and Learning:}}}
       
	   \REPEAT
	        \STATE{Search in $Memo$ for the  ($c_{close},y_{close}$) closest to ($c,y_g$)}
	        \STATE{ $mLow \gets$  mode $global-exploration$ or $local-optimization$ with probability   $\propto Sim((c,y_{close}),(c, y_g))$}
	  
	        \IF{ $mLow$ = $global-exploration$}
	        \STATE{Action parameter $a \gets$  random movement parameters}
	        \STATE{$y \gets $  \textsf{ Execute}($c, a$)}
	       \ELSIF{ $mLow$ =  $local-optimization$}
	     \STATE{\textsf{LocalOptimization}($c,y_g$) }
	  \ENDIF
	  \UNTIL{Terminate local exploration}

    \ELSE
	     \STATE{\textbf{\underline{High Level of Active Learning : Module 1 Social Learning}}}    
	       \REPEAT
	       \STATE{Ask the teacher for a demonstration $(c_{demo}, act_{demo},  y_{demo})$,  translate into movement parameters $a_{demo} \gets \textsf{ Correspondance}(act_{demo})$ }  
  \STATE{Set the goal $y_g \gets y_{demo}$ and the context $c \gets c_{demo}$ }
  \STATE {Select $R_n \in \mathcal{R}$ the region that contains $(c,y_{demo})$}
 % \STATE{EXECUTE $a_{demo}$}
        \STATE{{\underline{Low Level : Imitation:}}}
  	\FOR{$nbImitate$ times}
	\STATE{$a \gets a_{demo} + a_{rand}$ where $a_{rand}$ is a random vector such that $|a_{rand}|< \epsilon_{max}$ }
	\STATE{$y \gets $ \textsf{ Execute} ($c,a$)}
	\ENDFOR

	  \UNTIL{Terminate interaction with teacher}


\ENDIF

  \STATE{\textbf{\underline{High Level of Active Learning : Module 3 Goal Interest Computation}}}
\STATE{Compute the competence $\gamma_{y_g}$ }
\STATE{\textsf{UpdateRegions}($(c,y_g),\gamma_{y_g})$}
\STATE{\textsf{UpdateRegions}($(c,y),1), \forall y$ experienced in the loop}
\ENDLOOP	  


\end{algorithmic}
\end{algorithmbis}

==> SGIMACTSalgorithm/PseudoCodeSGIMACTS.tex <==
\begin{algorithmbis}[\textsf{SGIM-ACTS}]\label{alg:PseudoCodeSGIMACTS}
\begin{algorithmic}
\STATE  {\bfseries Input:} for $ \sigma_i=2 $ to $\sigma_{n}$ the different strategies. %($\sigma_1$ is intrinsic motivation).
\STATE  {\bfseries Initialization:} $\mathcal{R } \gets $  singleton $ Y$
\STATE  {\bfseries Initialization:} $Memo \gets$  empty episodic memory

\LOOP

\STATE{ $\sigma_i,\tau_i \gets \textsf{Select Task and Strategy}(c,\mathcal{R } )$}
  \IF{\underline{Mimic teacher $i$ strategy}}
  \STATE{ $ (\zeta_d,\tau_d) \gets$ ask and observe demonstration to teacher $i$. }
 % \STATE{\textsf{Emulation}: $\tau_g \gets \tau_{d}$ }%and the context $c \gets c_{demo}$ }
             \STATE{$\gamma_1 \gets$ Competence for $\tau_g$  }	
        \STATE{ Memo $\gets {\textsf{Imitate Action}} (\zeta_{d}$) }
            \STATE{$\gamma_2 \gets$ Competence for $\tau_g$  }

  \ELSIF{\underline{Emulate teacher $i$ strategy}}
  \STATE{ $ (\zeta_d,\tau_d) \gets$ ask and observe demonstration to teacher $i$. }
  \STATE{\textsf{Emulation}: $\tau_g \gets \tau_{d}$ }%and the context $c \gets c_{demo}$ }
             \STATE{$\gamma_1 \gets$ Competence for $\tau_g$  }	
    \STATE{ Memo $ \gets {\textsf{Goal-Directed Policy Optimisation}}(\tau_g) $}
            \STATE{$\gamma_2 \gets$ Competence for $\tau_g$  }

  \ELSE
  \STATE{ \textbf{\underline{Intrinsic Motivation strategy}}}
   \STATE{\ $\tau_g \gets \tau_{i}$ }%and the context $c \gets c_{demo}$ }
               \STATE{$\gamma_1 \gets$ Competence for $\tau_g$  }	
  \STATE{ Memo $ \gets {\textsf{Goal-Directed Policy Optimisation}}(\tau_g) $}
        \STATE{$\gamma_2 \gets$ Competence for $\tau_g$  }
\ENDIF

\STATE{$progress \gets  2*( sigmoid(\alpha_p* \frac{\gamma_2 -\gamma_1}{|T_i|*(nbActions tried)} -1 )$;  }
  \STATE{ $\mathcal{R } \gets $ Update $\textsf{Goal Interest Mapping}(\mathcal{R },Memo,y_g,progress)$}

\ENDLOOP	  
\end{algorithmic}
\end{algorithmbis}

==> SGIMACTSalgorithm/PseudoCodeSelectRegime.tex <==
\begin{algorithmbis}[$\textsf{[flagInter] = SelectStrategy}(\Delta_S,\Delta_A)$]\label{alg:PseudoCodeRegimeSelection}
\begin{algorithmic}
\STATE { {\bfseries input}:  $\Delta_S$ : progress values made by social learning strategy}
\STATE { {\bfseries input}:  $\Delta_A$ : progress values made by intrinsic motivation learning strategy}
\STATE { {\bfseries output}: $flagInter$ : chosen strategy}
\STATE { {\bfseries parameter}: $nbMin$ : duration of the initiation phase}
\STATE { {\bfseries parameter}: $ns$ : window frame for monitoring progress}
\STATE { {\bfseries parameter}: $cost$ : cost of requesting a demonstration}

\STATE{\textbf{\underline{Initiation phase}}}
\IF{ Social Learning and Intrinsic Motivation Regimes have not been chosen each $nbMin$ times yet}
\STATE{$ps \gets 0.5$}
\ELSE
\STATE{\textbf{\underline{Permanent phase}}}
\STATE{$wa \gets$ average(last $ns$ elements of $\Delta_A$)}
\STATE{$ws \gets \frac{average(\textsf{last }ns \textsf{elements of } \Delta_S)}{cost}$}
\STATE{ $ps \gets min(0.9, max(0.1, \frac{ws}{ws + wa} ))$}
\ENDIF

\STATE{flagInter $\gets$ true with probability $ps$}
\RETURN{flagInter}

\end{algorithmic}
\end{algorithmbis}

==> SGIMACTSalgorithm/PseudoCodeUpdateRegions.tex <==
\begin{algorithmbis}[\textsf{ [$\mathcal{R}$] = UpdateRegions}($\tau,progress, \sigma$) ] \label{alg:UpdateRegions}
\begin{algorithmic}
\STATE {\bfseries input:} $\mathcal{R}$: set of regions and corresponding $interest(\sigma)$ for each strategy $\sigma$.
\STATE {\bfseries input}: $g_{Max}$ : the maximal number of elements inside a region.
\STATE {\bfseries input:} $\delta$ : a time window used to compute the interest.
\STATE{Find the region $R_n \in \mathcal{R}$ such that $\tau \in R_n$.}
\STATE{Add $progress$ in $R_n(\sigma)$, the list of competence progress measures of experiments $ \tau \in R_n$ with strategy $\sigma$.}
\STATE{Compute the new value of  competence progress of $R_n(\sigma)$: } 
\begin{center}
\STATE{$interest_{R_n}(\sigma) =  \kappa (\sigma) \frac{ \displaystyle mean_{i=|{R}_n|-\frac{\delta}{2}}^{|{R}_n|} progress_{i} }{\delta}$}
\end{center}
\IF{ $|R_n(\sigma)| > g_{max}$}
\STATE{ $\mathcal{R} \gets$ Split $R_n$. }
\ENDIF
\RETURN $\mathcal{R}$
\end{algorithmic}
\end{algorithmbis}

